Baseline hydropower generation offer curves

We outline a mathematical model for pricing hydropower generation. The model involves a Markov decision process that reflects the seasonal variation in historical time series of water inflows. The procedure is computationally efficient and easy to interpret.

==> old-formulation.tex <==

We are now in a position to present the dual pair of optimization problems that can be solved to 1) optimize the overall system costs of utilizing a hydro reservoir in conjunction with other (e.g., thermal) resources, and faced with inflow (and possibly electrical demand) uncertainty, and 2) optimizing the plan of actions for operating the reservoir. 
In particular, any vector $(u^{\ast}, v^\ast)$ that solves the linear program 
\begin{equation}
    % \label{eq:val_max}
    \begin{array}{ll}
        \max_{u, \vec{v}} u & \\
         u + v_s \leq {}& c_{sa} + \sum_{s^\prime} p_{s^\prime|sa} v_{s^\prime} \quad  \forall s, a 
    \end{array}
    \end{equation}
provides the maximum expected value, or equivalently minimum expected cost of operating the integrated electricity system $u^{\ast}$ along with the optimum expected values/costs of the system in each state $s$, namely the components $v^{\ast}_s$ of vector $v^{\ast}$ (see e.g. \cite{bertsekas_2018v2}). Furthermore, \eqref{eqn:state-action-lp} formulated below provides the optimal action plan for governing the system. 
\begin{align}
    y^{\ast} \coloneqq {}& \arg\min_{y \in Y} \sum_{s, a} c_{sa} y_{sa}
        % \label{eqn:state-action-lp}
\end{align}
Recall that $ y_{sa}$ is the probability of being in state $s$ and executing action $a$, and we have 
\begin{align}
    \Delta \coloneqq {}& \{y \in \mathbb{R}^{S \times A}: ~ \sum_{a, s} y_{sa} = 1, ~ y \geq 0 \} 
        \label{eqn:simplex}
    \\
    Y \coloneqq {}& \{
        y \in \Delta: 
        \sum_a y_{s^\prime a} =
            \sum_{a, s} p_{s^\prime|sa} y_{sa} ~
        \forall s^\prime \in S
    \} 
        \label{eqn:markov}
\end{align}
\(\Delta\) is the set of valid probability distributions over state-action pairs, and \(Y\) is the subset compatible with the conditional transition probabilities specified in \(p\).
Note that \eqref{eqn:state-action-lp} is the dual problem to \eqref{eq:val_max}, therefore
by linear programming duality, \(u^\ast = c\cdot y^\ast\) is the expected cost per unit period of running the system according to the optimal policy \(y^ast\). The right-hand side of the constraint might be written as \(c_{sa} + \expect(v_{s^\prime} | s, a)\) combines the immediate cost of a single state transition \(s \overset{a}{\rightarrow} s^\prime\) with the expected downstream costs of subsequent actions.

While the formulation of \eqref{eqn:state-action-lp} yields a probabilistic plan of action (i.e., take action $a$ in state $s$ with probability $y^{\ast}_{sa}$), it can be shown that, in the absence of floating-point error, \(y^\ast\) has a single supported action for each state. 


